Large-Scale Image Retrieval with Attentive Deep Local Features

We propose an attentive local feature descriptor suitable for large-scale image retrieval, referred to as DELF (DEep Local Feature). The new feature is based on convolutional neural networks, which are trained only with image-level annotations on a landmark image dataset. To identify semantically useful local features for image retrieval, we also propose an attention mechanism for keypoint selection, which shares most network layers with the descriptor. This framework can be used for image retrieval as a drop-in replacement for other keypoint detectors and descriptors, enabling more accurate feature matching and geometric verification. Our system produces reliable confidence scores to reject false positives---in particular, it is robust against queries that have no correct match in the database. To evaluate the proposed descriptor, we introduce a new large-scale dataset, referred to as Google-Landmarks dataset, which involves challenges in both database and query such as background clutter, partial occlusion, multiple landmarks, objects in variable scales, etc. We show that DELF outperforms the state-of-the-art global and local descriptors in the large-scale setting by significant margins. Code and dataset can be found at the project webpage: https://github.com/tensorflow/models/tree/master/research/delf .

==> sections/metrics.tex <==
%!TEX root = ../iccv_main.tex

\section{Evaluation} \label{sec:metrics}
Image retrieval systems have typically been evaluated based on mean average precision (mAP), which is computed by sorting images in descending order of relevance and averaging accuracies for individual thresholds.
This evaluation method may be a reasonable choice in the existing datasets such as Oxford5k/105k~\cite{Philbin07}, Paris6k/106k~\cite{Philbin2008} and Holiday~\cite{Jegou2008} because there are no distractors in query (and database) and the sizes of the datasets are small.

However, for the case in large-scale datasets with a lot of queries including distractors, such evaluation method may not be representative since it is important to determine whether each image is relevant to the query or not and ranking irrelevant images is not interesting at all.
In addition, since the scales of scores may be different across query images, it is not straightforward to set a unified threshold to determine the relevance of each image to query, especially in the presence of distractors in dataset and query.

Therefore, we employ precision and recall information instead.
%In particular, we are interested in measuring the recall achieved at high precision operating points, for example, $\mathrm{Recall}@90\%$ (in short, $\mathrm{R}@90\%$).
Slightly different from the standard definitions of precision (\textsc{Pre}) and recall (\textsc{Rec}) per image, we consider all query images at the same time as in the following equations because recall is not well-defined for distractor queries:
\begin{align}
\textsc{Pre} = \frac{\sum_{q} | \mathcal{R}^\text{TP}_q |}{\sum_{q} |\mathcal{R}_i |}~~\text{and}~~
%\label{eq:precision}
%\textsc{Rec} = \frac{\sum_{q} | \mathcal{R}^\text{TP}_q |}{\sum_{q} | \mathcal{G}_p |}, \nonumber
\textsc{Rec} = \sum_{q} | \mathcal{R}^\text{TP}_q |,
%\label{eq:recall}
\label{eq:pr_def}
\end{align}
%where $\mathcal{R}_q$ and $\mathcal{G}_q$ denote a set of retrieved and ground-truth images for query $q$, respectively, and $\mathcal{R}_q^\text{TP} (\subseteq \mathcal{R}_q)$ is a set of true-positive images in the retrieval.}
where $\mathcal{R}_q$ denotes a set of retrieved images for query $q$, and $\mathcal{R}_q^\text{TP} (\subseteq \mathcal{R}_q)$ is a set of true-positive images in the retrieval.
%$| \cdot |$ means the size of a set.


\iffalse
The main application considered in our work is different from that of most existing image retrieval systems.
We discuss two variants of objectives for image retrieval tasks, and describe how we verify the effectiveness of the proposed algorithm in the context of our focus.

\subsection{Ranked vs. Unranked Image Retrieval}
Image retrieval applications can be broadly categorized into two types: (i) ranked retrieval, and (ii) unranked retrieval.
In the first case, systems return a list of results, ranked in descending order of relevance, so even loosely relevant items might be included in this list.
An example of this type of application is web image search, where a user's goal is often to explore potentially similar images to the query.
The performance metric commonly used in this case, mean average precision (mAP), does not penalize returning more results, even if they are incorrect.
%
%As a matter of fact, mAP cannot decrease as more results from a ranked list are returned.

In the second type of application, unranked retrieval, a system is expected to return only the items that are relevant for a given query.
%As an example, consider a system whose task is to assign landmark labels to photos from a personal collection.
%The system can either label the image as containing the landmark or not.
The relevance score of each item in the database may not be reported.
Usually, such systems must operate with high precision, in order to avoid exceeding a tolerable false positive rate.
In this setup, it is very important to effectively handle distractor queries, \ie, queries that have no relevant matches in the database, by simply not returning any result.
In this setting, the absolute scores of database images for a given query are important, as only the images with sufficiently high scores should be returned.
An example of this type of application is the automatic annotation of personal photos with landmark labels, where the system should only suggest annotations with high confidence.


\subsection{Performance Assessment}
Our main focus is the unranked image retrieval problem.
For proper evaluation of the target task, we measure the recall achieved at high precision operating points, for example, $\mathrm{Recall}@90\%$ (in short, $\mathrm{R}@90\%$).
%In the next section, we evaluate our proposed technique with this retrieval setup, and compare it against several recent image retrieval methods.
%
%As presented in \secref{sec:metrics}, our main focus is the unranked image retrieval setup, where systems are most commonly designed to operate with high precision.
To take distractor queries into account, precision and recall measures need to consider all queries together, since recall is not well-defined when evaluating retrieval results for a single distractor query.
More precisely, for a given threshold $\tau$ to accept a retrieval match, denote the number of retrieved results for query $q$ by $R_q$, the number of retrieved true positive results by $R^{TP}_q$, and the number of ground-truth true positive database images by $G_q$.
We compute precision ($\mathcal{P}$) and recall ($\mathcal{R}$) respectively as
\iffalse
\vspace{-25pt}
\begin{multicols}{2}
  \begin{equation}
	\mathrm{P} = \frac{\sum_{q=1}^{Q} R^{TP}_q}{\sum_{q=1}^{Q} R_q}
	\label{eq:precision}
  \end{equation}\break
  \begin{equation}
	\mathrm{R} = \frac{\sum_{q=1}^{Q} R^{TP}_q}{\sum_{q=1}^{Q} G_q},
	\label{eq:recall}
  \end{equation}
\end{multicols}
\fi
%
\begin{align}
\mathcal{P} = \frac{\sum_{q=1}^{Q} R^{TP}_q}{\sum_{q=1}^{Q} R_q}~~\text{and}~~
%\label{eq:precision}
\mathcal{R} = \frac{\sum_{q=1}^{Q} R^{TP}_q}{\sum_{q=1}^{Q} G_q}, \nonumber
%\label{eq:recall}
\end{align}
where $Q$ denotes the number of queries in the dataset.
\fi
